The Galactic population of magnetars : a simulation-based inference study

Population synthesis modeling of the observed dynamical and physical properties of a population is a highly effective method for constraining the underlying birth parameters and evolutionary tracks. In this work, we apply a population synthesis model to the canonical magnetar population to gain insight into the parent population. We utilize simulation-based inference to reproduce the observed magnetar population with a model which takes into account the secular evolution of the force-free magnetosphere and magnetic field decay simultaneously and self-consistently. Our observational constraints are such that no magnetar is detected through their persistent emission when convolving the simulated populations with the XMM-Newton EPIC-pn Galactic plane observations, and that all of the $\sim$30 known magnetars are discovered through their bursting activity in the last $\sim50$ years. Under these constraints, we find that, within 95 % credible intervals, the birth rate of magnetars to be $1.8^{+2.6}_{-0.6}$ kyr$^{-1}$, and lead to having $10.7^{+18.8}_{-4.4}$ % of neutron stars born as magnetars. We also find a mean magnetic field at birth ($\mu_b$ is in T) $\log\left(\mu_b\right) = 10.2^{+0.1}_{-0.2}$, a magnetic field decay slope $\alpha_d = 1.9 ^{+0.9}_{-1.3}$, and timescale $\tau_d = 17.9^{+24.1}_{-14.5}$ kyr, in broad agreement with previous estimates. We conclude this study by exploring detection prospects: an all-sky survey with XMM-Newton would potentially allow to get around 7 periodic detections of magnetars, with approximately 150 magnetars exceeding XMM-Newton's flux threshold, and the upcoming AXIS experiment should allow to double these detections.

==> tables/known_detections.tex <==
\begin{table}[]
    \centering
\begin{tabular}{c}

    \begin{tabular}{c|c}
         &  \\
         & 
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}{c}
    Magnetars: \\
    4U 0142+61, 0654870101 \\
    SGR 0501+4516, 0552971401 \\
    1E 1048.1-5937, 0723330101 \\
    1E 1547.0-5408, 0560181101 \\
    SGR 1806-20, 0152833001 \\
    SGR 1833-0832, 0605851901, in quiescence? \\
    1E 1841-045, 0783080101 \\
    SGR 1900+14, 0305580101 \\
    % 1E 2259+586, 0057540201 \\
    CXOU J164710.2-455216, 0555350101 \\
    1RXS J170849.0-400910, all obs in SmallWindow \\
    CXOU J171405.7-381031, 0670330101 \\
    SGR J1745-2900, 0700980101, likely not detectable in quiescence \\
    XTE J1810-197, 0720780301 \\
    Swift J1818.0-1607, 0823591801, likely not detectable in quiescence \\
    AX J1818.8-1559, 0823594001 \\
    Swift J1822.3-1606, 0722520101, likely not detectable in quiescence \\
    Swift J1834.9-0846, 0605851901, likely not detectable in quiescence \\
    \\
    
    Other detected sources: \\
    4U 0115+63: X-ray pulsar, 0804940201 \\
    J19294+1816: HMXB, 0841190101, \cite{bff+11}

\end{tabular}
